LOCO-EPI: Leave-one-chromosome-out (LOCO) as a benchmarking paradigm for deep learning based prediction of enhancer-promoter interactions

In mammalian and vertebrate genomes, the promoter regions of the gene and their distal enhancers may be located millions of base-pairs from each other, while a promoter may not interact with the closest enhancer. Since base-pair proximity is not a good indicator of these interactions, there is considerable work toward developing methods for predicting Enhancer-Promoter Interactions (EPI). Several machine learning methods have reported increasingly higher accuracies for predicting EPI. Typically, these approaches randomly split the dataset of Enhancer-Promoter (EP) pairs into training and testing subsets followed by model training. However, the aforementioned random splitting causes information leakage by assigning EP pairs from the same genomic region to both testing and training sets, leading to performance overestimation. In this paper we propose to use a more thorough training and testing paradigm i.e., Leave-one-chromosome-out (LOCO) cross-validation for EPI-prediction. We demonstrate that a deep learning algorithm, which gives higher accuracies when trained and tested on random-splitting setting, drops drastically in performance under LOCO setting, confirming overestimation of performance. We further propose a novel hybrid deep neural network for EPI-prediction that fuses k-mer features of the nucleotide sequence. We show that the hybrid architecture performs significantly better in the LOCO setting, demonstrating it can learn more generalizable aspects of EP interactions. With this paper we are also releasing the LOCO splitting-based EPI dataset. Research data is available in this public repository: https://github.com/malikmtahir/EPI

==> table7.tex <==
\begin{table*}[h]
	\centering
        \captionsetup{justification=centering}
	\caption{Tabular details of each layer in the proposed $M_{Hybrid}$ architecture.}
	
	\begin{adjustbox}{width=\textwidth,center}
        \begin{tabular}[t]{lll}
    \hline	
Layer                                & Output shape & Description                                                         \\
    \hline	

Input 1                              & (3000, 4)    & Input of   Enhancer                                                 \\
Input 3                              & (2000, 4)    & Input of Promoter                                                   \\
Conv1D(16,13,2)                      & (1500, 16)   & Convolution   layer of Enhancer                                     \\
Conv1D(32,23,2)                      & (1000, 16)   & Convolution   layer of Enhancer                                     \\
Conv1D) (16,13,2)                    & (750, 32)    & Convolution   layer of Promoter                                     \\
Conv1D) (32,23,2)                    & (500, 32)    & Convolution   layer of Promoter                                     \\
MaxPooling1D(size   =40, strides=20) & (36, 32)     & Max Pooling   layer for Enhancer                                    \\
MaxPooling1D(size   =40, strides=20) & (24, 32)     & Max Pooling   layer for Promoter                                    \\
Dropout(0.5)                         & (36, 32)      & Dropout layer   of Enhancer                                         \\
Input 2                              & (1, 1024)    & k-mer input   of Enhancer                                           \\
Dropout(0.5)                         & (24, 32)     & Dropout layer   for k-mer Enhancer                                  \\
Input\_4                             & (1, 1024)    & k-mer input   of Promoter                                           \\
Flatten                              & 1152         & Flatten the   output of Enhancer Dropout layer                      \\
Flatten                              & 1024         & Flatten the   output of Dropout layer for k-mer Enhancer            \\
Flatten                              & 768          & Flatten the   output of Promoter Dropout layer                      \\
Flatten                              & 1024         & Flatten the   output of Dropout layer for k-mer Promoter            \\
Concatenate                          & 2176         & Concatenate   the feature map of CNN and k-mer of Enhancer          \\
Concatenate                          & 1792         & Concatenate   the feature map of CNN and k-mer of Enhancer          \\
BatchNormalization                   & 2176         & BatchNormalization   for Enhancer features                          \\
BatchNormalization                   & 1792         & BatchNormalization   for Promoter features                          \\
Dropout(0.5)                         & 2176         & Dropout for Enhancer   features                                     \\
Dropout(0.5)                         & 1792         & Dropout for Promoter   features                                     \\
Concatenate                          & 3968         & Concatenate   the Dropout output of Enhancer and Promoter           \\
BatchNormalization                   & 3968         & BatchNormalization   of Concatenate output of Enhancer and Promoter \\
Flatten                              & 3968         & Flatten the   output of BatchNormalization layer                    \\
Dense(1)                             & 1            & probability of EPI           \\                                          
    \hline
 	\end{tabular}
	\label{table7}
 \end{adjustbox}
\end{table*}
